Exploring the Social Context of Collaborative Driving

The automation of the driving task affects both the primary driving task and the automotive user interfaces. The liberation of user interface space and cognitive load on the driver allows for new ways to think about driving. Related work showed that activities such as sleeping, watching TV, or working will become more prevalent in the future. However, social aspects according to Maslow's hierarchy of needs have not yet been accounted for. We provide insights of a focus group with N=5 experts in automotive user experience revealing current practices such as social need fulfillment on journeys and sharing practices via messengers and a user study with N=12 participants of a first prototype supporting these needs in various automation levels showing good usability and high potential to improve user experience.

==> notes.tex <==
\begin{comment}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.65\textwidth]{figures/s7.jpg}
        \subcaption{Screenshot of the application with one additional waypoint and no friend invited. The drawer is closed, on the right side is the button for communication.}
        \label{fig:app_screenshot_2}
    \end{subfigure}
        \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.65\textwidth]{figures/s8.jpg}
        \subcaption{Screenshot of the application with one additional waypoint and no friend invited. Drawer is opened to display more information.}
        \label{fig:app_screenshot}
    \end{subfigure}
    \caption{Screenshot of the applications.}
    \label{fig:all_screenshots}
    %\vspace{-5mm}
\end{figure}
\end{comment}


\begin{comment}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/boxplot_pssuq.pdf}
        \subcaption{PSSUQ scores}
        \label{fig:pssuq}
    \end{subfigure}
        \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/boxplot_sam_all.pdf}
        \subcaption{SAM scores}
        \label{fig:sam}
    \end{subfigure}
            \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.70\textwidth]{figures/pssuq_sys_use.pdf}
        \subcaption{System usefulness scores}
        \label{fig:pssuq_sys_use}
    \end{subfigure}
            \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=0.80\textwidth]{figures/navigation_vs_social.jpg}
        \subcaption{Hypothesized growing importance of fulfilled social needs in AVs}
        \label{fig:nav_vs_social}
    \end{subfigure}
    \caption{Scores of the experiment}
    \label{fig:all_scores}
    %\vspace{-5mm}
\end{figure}




\begin{marginfigure}
    \includegraphics[width=1.05\marginparwidth]{figures/boxplot_pssuq.pdf}
    \caption{PSSUQ scores}
    \label{fig:pssuq}
\end{marginfigure}


\begin{marginfigure}
    \includegraphics[width=1.05\marginparwidth]{figures/boxplot_sam_all.pdf}
    \caption{SAM scores}
    \label{fig:sam}
\end{marginfigure}


\begin{marginfigure}
    \centering
    \includegraphics[width=0.68\marginparwidth]{figures/pssuq_sys_use.pdf}
    \vspace{-2mm}
    \caption{System usefulness scores}
    \label{fig:pssuq_sys_use}
\end{marginfigure}


\begin{marginfigure}
    \centering
    \includegraphics[width=1.00\marginparwidth]{figures/navigation_vs_social.jpg}
    \caption{Hypothesized growing importance of fulfilled social needs in AVs}
    \label{fig:nav_vs_social}
\end{marginfigure}

\end{comment}


%\subsection{Participants}
\begin{comment}



\begin{table}[H]
\small
\begin{tabular}{p{0.2cm}|p{0.45cm}p{0.3cm}p{2.2cm}p{7.9cm}}
\centering
ID & Gender & Age & autoUX experience & Previous UX experience \\ \hline
P1 &  M     &  26 & 3 & UX and interface design for automotive UI and web-development\\ \hline
P2&  F     &  28 & 4 & design of: infotainment, apps, web; conception and specification \\ \hline
P3 &  F     &  26 & 1 & e-learning apps, web design, infotainment\\ \hline
P4 &  F     &  30 & 5 & none\\ \hline
P5 &  M     &  33 & 4 & technical specification of rear seat; infotainment HMI\\ 
\end{tabular}
\caption{Demographic information of focus group participants}
\label{table:participants_focus_group}
 \vspace{-4mm}
\end{table}
\end{comment}


%We recruited \N{5} participants (cf.~\autoref{table:participants_focus_group}). The experts were recruited via the company \textit{Elektrobit}~\cite{elektrobit} which is working on automotive user interface design.

\begin{comment}

\begin{marginfigure}
    \includegraphics[width=1.05\marginparwidth]{figures/focus_group.jpg}
    \caption{Focus group setup}
    \label{fig:focus_group}
\end{marginfigure}

\end{comment}

\begin{comment}
\begin{marginfigure}
    \includegraphics[width=\marginparwidth]{figures/apparatus_2_crop_number.JPG}
    \caption{Study setup: mic (1) and app (2).}
    \label{fig:apparatus}
\end{marginfigure}
\end{comment}
